Alchemist: Towards the Design of Efficient Online Continual Learning System

Continual learning has become a promising solution to refine large language models incrementally by leveraging user feedback. In particular, online continual learning - iteratively training the model with small batches of user feedback - has demonstrated notable performance improvements. However, the existing practice of separating training and serving processes forces the online trainer to recompute the intermediate results already done during serving. Such redundant computations can account for 30%-42% of total training time. In this paper, we propose Alchemist, to the best of our knowledge, the first online continual learning system that efficiently reuses serving activations to increase training throughput. Alchemist introduces two key techniques: (1) recording and storing activations and KV cache only during the prefill phase to minimize latency and memory overhead; and (2) smart activation offloading and hedging. Evaluations with inputs of varied token length sampled from ShareGPT dataset show that compared with a separate training cluster, Alchemist significantly increases training throughput by up to 1.72x, reduces up to 47% memory usage during training, and supports up to 2x more training tokens - all while maintaining negligible impact on serving latency.

==> Makefile <==


# generate main.pdf via pdflatex
pdf:
	pdflatex main.tex
	pdflatex main.tex

# by default 
all: pdflatex

# quick compile
q:
	latex main.tex

# second quick conmpile
qq: todvi

# generate the dvi
todvi:
	latex main.tex
	bibtex -min-crossrefs=100 main
	latex main.tex
	latex main.tex

# open the main.dvi
x:
	xdvi -bg white main.dvi &


# compile full and open the pdf
p: todvi tops topdf open cleanabit 

# generate the main.ps
tops:
	dvips -o main.ps main

# generate the main.pdf
topdf:
	ps2pdf14 main.ps

# open the pdf
open:
	${HOME}/bin/pdfreader main.pdf

# cleaning a bit
cleanabit:
	rm -vf *~ *.ps  *.aux *.log \
	*.bbl *.blg *.out *.brf *.4*  \
	*.css *.idv *.lg *.tmp *.xref *.png *.toc

# clean
clean: cleanall clean-eps-converted-pdf

# clean all
cleanall:
	rm -vf *.ps  main.pdf *.dvi *.aux *.log \
	*.bbl *.blg *.out *.brf *.4*  \
	*.css *.idv *.lg *.tmp *.xref *.png *.toc \
	*.synctex.gz *.fdb_latexmk *.fls *.synctex\(busy\) *.synctex.gz\(busy\) \
	*.pdf

# clean eps-converted-pdf
clean-eps-converted-pdf:
	find F/ -name "*eps-converted-to.pdf" -exec rm -fv  '{}' \;



==> fig-empty.tex <==

\begin{figure}[h]
  \centering
  \includegraphics[]{}
  \mycaption{}{Short caption}{Long caption}
\end{figure}



==> fig-prefetch.tex <==

\begin{figure}[h]
  \centering
  \includegraphics[]{}
  \mycaption{Short caption}{Long caption}
\end{figure}



==> motiv-cont-learn.tex <==
\subsection{Continuous Learning}%
\label{motiv-cont-leanr}

In many real-world applications, it is crucial to continually adapt models to
new data or user feedback to remain performant. This paradigm, often referred
to as {\em continuous learning} (CL), allows a system to learn incrementally
by incorporating feedback or additional information collected during usage.

\mypara{Continual Pretraining}
One dimension of continuous learning addresses the need for continual
pretraining on the latest, dynamically changing information. This scenario aims
to keep the knowledge base of the model current. Here, user prompts, search
contexts, and real-time content (\eg~news, finance data, emerging social media
trends) feed into the continual pretraining pipeline. Fields like finance,
fashion, and journalism, where timeliness is critical, can benefit greatly from
this mechanism. As new market data arrives or trending topics emerge, the model
incorporates this fresh information into its pretrained representations,
ensuring that subsequent responses better reflect current realities.

\mypara{Continual Preference Alignment}
Beyond merely updating knowledge, many applications also require continuously
aligning model outputs with either users' new preference or emerging new
users' preference. Techniques such as {\em Direct Preference Optimization
    (DPO)}~\cite{xxx} and its derivative methods have emerged as the go-to
strategies for preference alignment. This trend is due to their ability to
align the model {\em directly} with user feedback based on a simple binary
preference (\ie~like and dislike), rather than a complex and possibly unstable
reward model in prior Reinforcement Learning with Human Feedback (RLHF)
methods.

A pervasive example where preference alignment can be used to approve models
is for the tools like code-writing assistants (\eg~Copilot in VSCode) or a
grammar correction tool (\eg~Grammarly). For this type of tools, based on the
users' previous input text, the model will prompt its generated text/code as a
suggestion. Users then have the choice of accepting or not accepting the
suggestions. This accepting or rejecting behavior will be treated as the
preference label. If the user accepts the suggestion, it means the user likes
the output. If not, the user can continue to type, and user's input afterward
can be treated as this user's preferred text/code.

DPO and its derivatives can also be applied even if users do not explicitly
provide their preferred text. For example, in a chatbox application, users can
like or dislike the creativity in the generation output. If the user dislikes
the creativity, when training, we can the same user prompts but now prefixing
with the instruction to lower the creativity in generation (\eg~"Please do not
be creative..."). We can then use the text generated with new instruction as
this user's preferred text.


==> motiv-fm.tex <==
\subsection{Foundation Model}%
\label{motiv-fm}

Foundation models (FM) are a type of large-scale and pretrained machine
learning model trained on massive datasets from a wide spectrum of sources. FM
are typically trained for general purposes, and, hence, can be used as the
backbone of a variety of downstream applications. Transformers, due to their
ability to scale up to huge amounts of parameters, are often used as FMs to
learn from general-purpose corpus, and {\em fine-tuned} on more specific
datasets for different specific AI applications' needs. For example, an FM can
be fine-tuned on a corporation's internal code base to provide tailored code
auto-completion or bug-detection.

% % However, since directly
% % deploying an FM may not satisfy every single application's needs, it is common
% % for AI applications developers to {\em fine-tune} an FM on smaller but more
% % specific datasets for their specific service needs. 
% For instance, A
% code-oriented FM (\eg~one trained with GitHub public repositories) can be
% fine-tuned on an organization’s internal private codebases to provide more
% tailored auto-completion or bug-detection for internal developers.


==> motiv-intro.tex <==
\section{Background \& Motivation}%
\label{motiv-intro}



==> motiv-model-train.tex <==
\subsection{Model training basics}%
\label{motiv-model-train}

A model training loop mainly consists of two parts: a forward pass and a
backward pass (or backpropagation). During the forward pass, the input is
passed through the model layer by layer to compute a final prediction, $y$.
Within each layer, the input is transformed by several linear operations (\eg,
matrix or vector multiplication) followed by a nonlinear operation (\eg,
$tanh(x)$), commonly referred to as the {\em activation function}. The
intermediate results from these activation functions, called {\em
activations}, are then passed to the next layer as input.

Next, the backward pass aims to minimize the difference between the model
prediction $y$ produced from forward pass and the ground truth $\hat{y}$. To
do this, it relies on a loss function $l$ that quantifies the difference
between the prediction and the ground truth. To determine how to update the
model weights so as to minimize the loss (\ie, reduce this difference), the
backward pass calculates the gradients by taking the derivatives of the loss
with respect to the model weights. In each iteration of the training loop, the
model weights are then updated in a small step along these gradients, thereby
iteratively reducing and eventually minimizing the loss.

To ensure efficiency, we often {\em store the activations} computed during the
forward pass for use in backpropagation. For example, suppose the forward pass
computes an activation $a = f(x)$, followed by a linear operation with model
weights $w_1$, yielding the prediction $y = a = f(x\cdot w_1)$. If, for the
simplicity of demonstration, we use the numerical difference between $y$ and
$\hat{y}$ as the loss function, we have $L = a - \hat{y}$. During
backpropagation, the gradient of the loss with respect to $w$ is
$\frac{\partial a}{\partial w_1}\cdot a$ by chain rule.
Because $a$ was already computed during the forward pass, it is intuitive to {\em store this activation} rather than recompute it during backpropagation, thus avoiding redundant computation cost.
The process is further illustrated in Fig. \ref{fig-forward-backward}.

\input{fig-forward-backward}

==> motiv-transformers.tex <==
\subsection{Transformers Basics}%
\label{motvi-transformers}

Transformers~\cite{transformers} have become one of the most popular model
architectures in the recent wave of generative AI.

At a high level, a transformer takes a series of input tokens \footnote{A
``token'' can be a punctuation, a word, or a part of a word. Tokenizing an
input is much faster than the generation process.} and auto-regressively
generates a sequence of output tokens through two phases.

During the prefill phase, the model processes the series of input tokens at
once, by using the attention module in each of the $l$ layers. Finally, it
produces two three-dimensional tensors, including a key (K) tensor and a value
(V) tensor. These K and V tensors capture the semantic information in the
input tokens, which are called the {\em KV cache}.

During the token-generation phase, also called decoding phase, the KV cache
produced at the prefill phase is used to compute the attention score between
the newly generated tokens with tokens in the input, and generate output
tokens one-by-one.

